Function-Correcting Codes

In this paper we study function-correcting codes, a new class of codes designed to protect the function evaluation of a message against errors. We show that FCCs are equivalent to irregular-distance codes, i.e., codes that obey some given distance requirement between each pair of codewords. Using these connections, we study irregular-distance codes and derive general upper and lower bounds on their optimal redundancy. Since these bounds heavily depend on the specific function, we provide simplified, suboptimal bounds that are easier to evaluate. We further employ our general results to specific functions of interest and compare our results to standard error-correcting codes, which protect the whole message.

==> introduction.tex <==
In standard communication systems, a sender desires to convey a digital message to a receiver via an erroneous channel. To protect this message from errors, the transmitter first encodes the message with an error-correcting code and then transmits the result over the channel. The receiver decodes the received word to obtain the original message. Classically, each part of the message is of equal importance to the receiver and the common goal is to construct a code with a suitable decoder such that the whole message can be recovered correctly.

Consider now the scenario where a certain \emph{attribute} of the message, i.e., the result of evaluating a certain function on the message, is of particular interest to the receiver. Assuming that the sender is aware of this function, she can encode the message such that the desired attribute is protected against errors. This paradigm gives rise to a new class of codes, which we call \emph{\fccs} (FCCs)\smallfalse. Such codes map a message to a codeword so that the recovery of a specific attribute, or function evaluation, of this message is possible, even in the presence of possible errors from the channel.
In this work we consider \emph{systematically encoded} codes where the original message itself is  transmitted over the channel, followed by redundant symbols from the~\fcc, see Fig.~\ref{fig:intro_fcc_problem}. 

\begin{figure}[t]
	\centering
	\begin{tikzpicture}[>=stealth]
		\node (u) {\u};
		\node[right = 0.5cm of u, rectangle, rounded corners, fill=gray!20!, draw, minimum height=0.75cm] (enc) {Encoder};
		\node[above left = 0.25cm and -0.5cm of enc] (alice) {\bfseries\large{Alice}};
		
		
		\node[draw,rectangle, rounded corners, fill=gray!20!, right = 1 cm of enc, minimum height=0.75cm] (channel) {Channel};
		\node[draw,rectangle, rounded corners, fill=gray!20!, right = 1 cm of channel, minimum height=0.75cm] (decoder) {Decoder};
		
		\node[below = 0.5cm of channel] (fu) {$f$};
		
		\node[right = 0.5cm of decoder](fy) {$f(\u)$};
		\node[above right= 0.25cm and -0.5cm of decoder] (bob) {\bfseries\large{Bob}};
		
		\draw[->] (u) -- (enc);%
		\draw[->] (enc) -- node [above] {$(\u,\p)$} (channel);
		\draw[->] (channel) -- node [above] {$\y$} (decoder);
		\draw[->] (decoder) -- (fy);
		\draw[->, dashed] (fu) -| (enc);
		\draw[->, dashed] (fu) -| (decoder);
	\end{tikzpicture}

	\caption{Illustration of the systematic \fcc\ setup. Alice has a message $\u$, which features an attribute $f(\u)$ that is of special interest to Bob. To guarantee recoverability of this attribute, Alice encodes the message $\u$ to a codeword $\c=(\u,\p)$. Given an erroneous version $\y$ of the codeword $\c$ and the knowledge of the function $f$, Bob can correctly infer $f(\u)$.}
	\label{fig:intro_fcc_problem}
\end{figure}%


The generic goal when designing \fccs\ for a given function is to use the smallest possible number of redundant symbols that allow the recovery of the attribute, given the received word. In principle, function-correction can be realized by protecting the full message against errors. This is because if the receiver is able to recover the message, he can evaluate the function on the message to obtain the desired attribute. %
However, due to the bottleneck property of function evaluations, it is clear that it is more efficient to protect only the specific function value of interest, especially when the message is long and the function image is small. Another direct construction of {\fccs} can be obtained by encoding the attribute with a standard error-correcting code and appending the result as the redundancy symbols. However, this solution ignores the side information brought by the original message. An efficient solution thus leverages this side information to potentially reduce the redundancy during the transmission.




A key aspect for the design of \fccs~is the topology of the function regions, i.e., the sets of message vectors that evaluate to the same function value. Since \fccs~protect a specific function evaluation on the message, the receiver does not need to be able to distinguish between codewords from messages that evaluate to the same function value. This means that the distance between any two codewords within one function region is irrelevant. On the other hand, codewords corresponding to different function values should have appropriate distance. Consequently, the redundancy vectors of an \fcc~have to fulfill an irregular distance profile, where each pair of redundancy vectors has to satisfy an individual distance constraint. This profile is defined by the function regions and the distances of the corresponding message vectors.










		
			
			






\fccs~have a natural connection to codes that admit unequal error protection. This connection manifests in the two levels of protection that \fccs\ provide to the message and the attribute. Since the message can either be unprotected or can itself be the codeword of an error-correcting code and the attribute is separately protected by the \fcc, it is possible to control the amount in which both these parts are protected against errors. As the attribute is the evaluation of an arbitrary function on the message, it is also possible that it is simply a substring of the message, resulting in unequal error protection for this part of the message. In general however, the attribute can be an arbitrary function of the message, meaning that \fccs~form a more general class of codes in this aspect.




{\em Related works:}

Unequal error protection codes \cite{masnick_linear_1967,boyarinov_linear_1981} assign to each message bit an individual error protection level and thus allow to protect specific parts of the message better than others. While similar on an abstract level, the irregular-distance codes in this paper require different levels of protection between specific messages, as opposed to specific message bits and thus the code design in this paper requires different techniques. For an information-theoretic study of both these classes of codes, we refer the reader to \cite{borade_unequal_2009}.

In the context of random access memories, codes with unequal message protection have been designed in \cite{schoeny_context-aware_2019}. The authors construct codes that guarantee larger distances for codewords that stem from a specific predefined subset of messages. Similarly to our work, the required distance varies between pairs of codewords. However, in \cite{schoeny_context-aware_2019}, the distance requirement only depends on the message groups to which the codewords are assigned, and here, as we will show later, we require an individual distance for each pair of codewords.

Another related line of work \cite{ahlswede_get_1981,orlitsky_coding_2001,kuzuoka_distributed_2016} studies the scenario, where a sender wishes to communicate a message to a receiver such that the receiver can determine the evaluation of a function on their combined data. Therein, optimal transmission rates for which the recovery of the function evaluation is possible, are derived. There are several important aspects that differentiate our work from these papers. First, we study zero-error codes over an adversarial channel as opposed to non-zero, but vanishing error probabilities. Second, the message sent from Alice to Bob may contain errors in our setup. Notice however that \cite{orlitsky_coding_2001} uses a characteristic graph \cite{witsenhausen_zero-error_1976}, which is similar in spirit to the irregular-distance codes defined later.


Codes that protect the output of a given machine learning algorithm against errors have been investigated in in~\cite{mazooji_robust_2016,kabir_coded_2017,huang_functional_2020-1}. While \cite{mazooji_robust_2016,kabir_coded_2017} tailored their construction to optimize classification algorithms, \cite{huang_functional_2020-1} applied codes to the weights of the neurons in a neural network with the goal to optimize the output model of the neural network. These works prove that application-specific codes that protect the output of an algorithm against errors can outperform classical error-correcting codes. In principle, we follow a similar idea in this work, however the research in \cite{mazooji_robust_2016,kabir_coded_2017,huang_functional_2020-1} is specialized to specific classes of functions, while we discuss arbitrary functions. On the other hand, with the current state of research, it seems infeasible to practically and efficiently apply our generic results to such intricate functions.


We further would like to highlight the following works on error-correction within computations. Fourier stabilization has been used in~\cite{raviv_enhancing_2021} to increase the robustness of a neural network. Therein, error resilience was achieved by replacing the weights of neurons according to the solution of an associated combinatorial optimization problem. In~\cite{roth_fault-tolerant_2019,roth_analog_2020,dupraz_noisy_2020} computation in faulty dot-product engines is treated. While \cite{roth_fault-tolerant_2019,roth_analog_2020} construct codes over integers and real numbers that protect the computation of a matrix-vector product, \cite{dupraz_noisy_2020} propose a theoretical framework for the error analysis of memristor crossbars.
Codes that correct and detect errors in arithmetic operations are discussed in~\cite[ch. 10]{lint_introduction_1999}. 

{\em Application:} The employment of \fccs\ can, for example, be beneficial in archival data storage. Assume a large data set, or message in our terminology, contains an attribute with highly sensitive information, which can be modeled as a function evaluation on the data set.
As the data set itself shall be accessible to all users, it must be directly stored on the archive, which motivates the discussion of systematic codes. On the other hand, due to the importance of the peculiar attribute, it is desirable to additionally protect it against errors. \fccs\ thus provide an individual level of protection to specific attributes of the message, offering higher flexibility and efficiency over classical error-correcting codes.

{\em Contributions:} This paper builds a general theory for function-correction over adversarial channels. For arbitrary functions, we establish a connection between \fccs\ and \emph{irregular-distance codes}. In particular, we show that the redundancy of an \FCC\ %
is given by the shortest length of an irregular-distance code, which has a punctured pair-wise distance profile, which depends on the function. Deriving general lower and upper bounds on the optimal length of irregular distance codes, we obtain corresponding bounds on the optimal redundancy of \fccs\ for arbitrary functions. These results are applied to specific functions such as locally binary functions, the Hamming weight, the Hamming weight distribution, the min-max function and functions that discretize real-valued functions. Finally, the redundancy of \fccs\ for specific functions is compared to schemes that use standard error-correcting codes. We
restrict our attention to binary channels in this work,
however most results can be generalized straightforwardly to
larger alphabets. A summary of our quantitative results for specific functions is summarized and displayed in Table \ref{tab:redundancy}.



{\em Organization:} Section~\ref{sec:prelim} summarizes the problem considered and the main notations of the paper. In Section~\ref{sec:irregular}, irregular-distance codes are introduced and generic upper and lower bounds on their optimal length are derived. Next, we show in Section~\ref{sec:generic} how to build {\fccs} using irregular distance codes. We first relate the optimal redundancy of an {\fcc} to the smallest length of an irregular-distance code and then provide simplified results that are easier to evaluate, especially for functions with entwined function regions. We then apply our generic results to specific functions in Sections~\ref{sec:locally_binary}, \ref{sec:hamming}, \ref{sec:min_max} and~\ref{sec:ml_functions}. Section~\ref{sec:conclusion} concludes the paper.

